TracLLM: A Generic Framework for Attributing Long Context LLMs

Long context large language models (LLMs) are deployed in many real-world applications such as RAG, agent, and broad LLM-integrated applications. Given an instruction and a long context (e.g., documents, PDF files, webpages), a long context LLM can generate an output grounded in the provided context, aiming to provide more accurate, up-to-date, and verifiable outputs while reducing hallucinations and unsupported claims. This raises a research question: how to pinpoint the texts (e.g., sentences, passages, or paragraphs) in the context that contribute most to or are responsible for the generated output by an LLM? This process, which we call context traceback, has various real-world applications, such as 1) debugging LLM-based systems, 2) conducting post-attack forensic analysis for attacks (e.g., prompt injection attack, knowledge corruption attacks) to an LLM, and 3) highlighting knowledge sources to enhance the trust of users towards outputs generated by LLMs. When applied to context traceback for long context LLMs, existing feature attribution methods such as Shapley have sub-optimal performance and/or incur a large computational cost. In this work, we develop TracLLM, the first generic context traceback framework tailored to long context LLMs. Our framework can improve the effectiveness and efficiency of existing feature attribution methods. To improve the efficiency, we develop an informed search based algorithm in TracLLM. We also develop contribution score ensemble/denoising techniques to improve the accuracy of TracLLM. Our evaluation results show TracLLM can effectively identify texts in a long context that lead to the output of an LLM. Our code and data are at: https://github.com/Wang-Yanting/TracLLM.

==> preliminary.tex <==
\section{Problem Formulation}
%We consider two parties: \emph{RAG system provider} and \emph{user}. The RAG system provider (e.g., XXX, XXX, XX) deploys its RAG system



\subsection{Problem Definition for Knowledge Tracing}
%Suppose$\mathcal{R}(Q)=\{T^1, T^2, \cdots, T^k\}$ is a set of $k$ retrieved texts for $Q$ from the knowledge database of RAG system. Given the $k$ retrieved texts $\mathcal{R}(Q)$ as the context, we use $A$ to denote the answer generated by the LLM in RAG. Our goal is to track back to the source of the answer $A$. To this end, we first define four potential modes:
Suppose $\mathcal{I}$ is the instruction of an LLM-based system. For instance, $\mathcal{I}$ can be ``Please answer the following question based on the provided context. Question: Who is the CEO of OpenAI? Context: [retrieved documents]'' in RAG systems; $\mathcal{I}$ can be ``Does this applicant have more than 5 years of Python experience? Answer yes or no.
Resume: [text of resume]'' in an LLM-integrated application for automated screening of applicants. We use $\mathcal{T}=\{T_1, T_2, \cdots, T_n\}$ to denote the $n$ texts of the input data. For instance, $T_i$ can be a retrieved document for a question in RAG systems. $T_i$ can be a document, a paragraph, a sentence, or a segment of text for LLM-integrated applications. We use $f$ to denote the LLM in an LLM-based system. Given the instruction $\mathcal{I}$ and the data $\mathcal{T}$, we use $O$ to denote the output of the LLM $f$ when taking $\mathcal{I}$ and $\mathcal{T}$ as input. 

 


\begin{definition}[Knowledge-Tracing Problem]
Suppose we have an instruction $\mathcal{I}$ and data $\mathcal{T} =\{T_1, T_2, \cdots, T_n\}$ with $n$ texts. We use $O$ to denote the output of the LLM $f$ in an LLM-based system when taking $\mathcal{I}$ and $\mathcal{T}$ as input. Knowledge tracing aims to find a subset of $K$ texts that make the most contribution for the LLM $f$ in generating $O$. Additionally, a ranking of these $K$ texts are provided based on their contribution.
    %Suppose we have a RAG system with the knowledge database $\mathcal{D}$ and the LLM $f$. Given a question $Q$, $\mathcal{R}(Q)=\{T^1, T^2, \cdots, T^k\}$ is a set of $k$ retrieved texts for $Q$ from $\mathcal{D}$. Suppose $A$ is the answer generated by the LLM for $Q$ with $k$ retrieved texts as the context. We aim to categorize the answer generation into one of the four potential modes (i.e., LLM, Context, LLM-Context-Independent, LLM-Context-Joint), i.e., 
\end{definition}
In our above definition, $K$ is a hyper-parameter that can be arbitrarily chosen by a user. For instance, user can set $K$ to be $n$. \RG{In this case, the problem becomes the standard feature attribution problem, where a ranking of all the $n$ texts in contributing to the output $O$ generated by $f$ is provided. However, as $n$ grows large, a ranking of all the $n$ texts becomes computationally inefficient and uninterpretable.} In this case, a knowledge-tracing framework will provide a ranking of the $n$ texts in contributing to the output $O$ generated by $f$. In many real-world scenarios, only a few paragraphs or sentences in a long document contributed to the output $O$. Thus, a user can also set a small $K$ to find a set of most important texts for $O$ in practice, thereby simplifying manual verification and saving computation costs. 

\myparatight{Design goals}
We aim to develop a knowledge-tracing framework for the knowledge-tracing problem. We have three goals in our design: \emph{efficient}, \emph{accurate}, and \emph{general}. Additionally, when our framework is used to identify malicious texts in adversarial settings, we also aim to achieve \emph{robustness} goal. Under mild assumptions, we prove that it is infeasible for an attacker to craft malicious texts that simultaneously mislead an LLM to generate attacker-desired output and prevent our knowledge-tracing framework from detecting these malicious texts.  

 

\subsection{Real-world Applications}
We discuss how our knowledge-tracing framework can be used to enhance the trustworthiness of long context LLM-based systems. 

\myparatight{Debugging LLM-based systems}Our knowledge tracing framework can be used as a tool to ``debug'' an LLM-based system. Take RAG systems as an example. Support an LLM in a RAG system generates an incorrect answer to user questions, where the incorrect answer can be reported by users or discovered by developers when debugging or testing RAG systems. Our framework can effectively pinpoint the most important retrieved texts that are responsible for the incorrect answers. 
In a recent indicient~\cite{}, Google Search with AI Overviews suggested adding glue to the sauce for a question on ``how to get cheese to stick to pizza''. Our method can automatically pinpoint the Reddit comment that leads to the undesired answer.  

\myparatight{Conducting post-attack forensic analysis}
Our framework can be used as a tool to conduct post-attack forensic analysis. In particular, our framework can automatically identify malicious texts after detecting attacks for an LLM-based system. For instance, an attacker can perform prompt injection attacks, which inject malicious instructions into the input data of an LLM-based system. Suppose a detection-based defense~\cite{} is deployed to detect whether the data input contains malicious instructions or not. After the detection, our framework can automatically pinpoint the malicious instructions in the input, which can greatly save labor costs, especially when data consists of many tokens.  
%In our evaluation, we show our framework can effectively identify malicious texts injected by an attacker to mislead an LLM to generate incorrect answers in RAG systems. 

\myparatight{Highlighting knowledge source for answers}LLM-based systems such as RAG, Agent, and LLM-Integrated applications can provide answers to user questions based on the input data. Our framework can highlight the most important paragraphs or sentences that provide supporting evidence for generated answers, which enables users to verify the source for the answers, thereby improving the trust of users towards the systems. 

\myparatight{More scenarios}
Our framework can also be used in many other scenarios such as 
